Lessons Learned from Data-Driven Building Control Experiments: Contrasting Gaussian Process-based MPC, Bilevel DeePC, and Deep Reinforcement Learning

This manuscript offers the perspective of experimentalists on a number of modern data-driven techniques: model predictive control relying on Gaussian processes, adaptive data-driven control based on behavioral theory, and deep reinforcement learning. These techniques are compared in terms of data requirements, ease of use, computational burden, and robustness in the context of real-world applications. Our remarks and observations stem from a number of experimental investigations carried out in the field of building control in diverse environments, from lecture halls and apartment spaces to a hospital surgery center. The final goal is to support others in identifying what technique is best suited to tackle their own problems.

==> CDC-2022 - Contrasting Data-Driven Techniques/data/Hospital.tex <==
\definecolor{myblue}{rgb}{0.20, 0.6, 0.78}
\definecolor{mygreen}{rgb}{0.2,0.8,0.2}
\definecolor{myred}{rgb}{0.5,0,0}
\definecolor{myorange}{HTML}{e28743}
 \begin{figure}
    \centering
    \begin{tikzpicture}
    \begin{axis}[
    date coordinates in=x,
    % date ZERO=2021-05-13 00:00,   % <-- needs to be set for v1.12 and below
    xmin=2021-11-12 00:08,
    xmax=2021-11-13 23:58,
    % set `xtick distance' to 3 hours (3/24)
    xtick distance=0.3,
    % set the label style of the `xtick's
    % xticklabel=\year.\month.\day\ \hour:\minute]
    xticklabel=\empty,
    % xmin=1, xmax=102,
    ymin=17.5, ymax= 21.1,
    enlargelimits=false,
    clip=true,
    grid=major,
    mark size=0.5pt,
    width=1.05\linewidth,
    height=0.45\linewidth,
    ylabel = {Indoor temperature [$^{\circ} C$]},
    % xlabel= time,
    ylabel style={at={(axis description cs:0.08,0.5)}},
    xlabel style={at={(axis description cs:0.5,0.05)}},
    legend columns=4,
    label style={font=\scriptsize},
    ticklabel style = {font=\scriptsize},
    legend style={
    	font=\footnotesize,
    	draw=none,
		at={(0.5,1.03)},
        anchor=south
    }    
    ]
    
    \pgfplotstableread[col sep=comma]{data/hospital.dat}{\dat}

    \addplot+ [ultra thick,smooth, mark=none, mark options={fill=white, scale=1,line width = 0.1pt},myred] table [x={t}, y={y1}] {\dat};    
    \addlegendentry{Room 1}
    \addplot+ [ultra thick,smooth, mark=none, mark options={fill=white, scale=1,line width = 0.1pt},myorange] table [x={t}, y={y2}] {\dat};    
    \addlegendentry{Room 2}
    \addplot+ [ultra thick,smooth, mark=none, mark options={fill=white, scale=1,line width = 0.1pt},myblue] table [x={t}, y={y3}] {\dat};    
    \addlegendentry{Room 3}    
    \addplot+ [name path =A, ultra thin, gray,draw opacity=0.6,mark = none] table [x={t}, y expr=\thisrow{mode}*150] {\dat};
    \addplot+ [name path =B, ultra thin, gray,draw opacity=0.6,mark = none] table [x={t}, y expr=\thisrow{mode}*-100] {\dat};
    \addplot[gray,fill opacity =0.15] fill between[of=A and B]; 
    
    
    
    \addplot+ [thick,brown,dashed,mark = none] table [x={t}, y={ymax}] {\dat};
    \addlegendentry{Constraint}     
    
    \end{axis}
    \end{tikzpicture}\\
    \begin{tikzpicture}
    \begin{axis}[
    date coordinates in=x,
    % date ZERO=2021-05-13 00:00,   % <-- needs to be set for v1.12 and below
    xmin=2021-11-12 00:08,
    xmax=2021-11-13 23:58,
    % set `xtick distance' to 3 hours (3/24)
    xtick distance=0.3,
    % set the label style of the `xtick's
    % xticklabel=\year.\month.\day\ \hour:\minute]
    xticklabel=\month.\day\ \hour {h},
    % xmin=1, xmax=102,
    ymin=39, ymax= 91,
    enlargelimits=false,
    clip=true,
    grid=major,
    mark size=0.5pt,
    width=1.05\linewidth,
    height=0.45\linewidth,
    ylabel = {Valve position [degs]},
    % xlabel= time,
    ylabel style={at={(axis description cs:0.08,0.5)}},
    xlabel style={at={(axis description cs:0.5,0.05)}},
    legend columns=4,
    label style={font=\scriptsize},
    ticklabel style = {font=\scriptsize},
    legend style={
    	font=\footnotesize,
    	draw=none,
		at={(0.5,1.03)},
        anchor=south
    }    
    ]
    
    \pgfplotstableread[col sep=comma]{data/hospital.dat}{\dat}

    \addplot+ [thick,const plot, mark=none, mark options={fill=white, scale=1,line width = 0.1pt},myred] table [x={t}, y={u1}] {\dat};    
    % \addlegendentry{Room 1}
    \addplot+ [thick,const plot, mark=none, mark options={fill=white, scale=1,line width = 0.1pt},myorange] table [x={t}, y={u2}] {\dat};    
    % \addlegendentry{Room 2}
    \addplot+ [thick,const plot, mark=none, mark options={fill=white, scale=1,line width = 0.1pt},myblue] table [x={t}, y={u3}] {\dat};    
    % \addlegendentry{Room 3}    
    \addplot+ [name path =A, ultra thin, gray,draw opacity=0.6,mark = none] table [x={t}, y expr=\thisrow{mode}*150] {\dat};
    \addplot+ [name path =B, ultra thin, gray,draw opacity=0.6,mark = none] table [x={t}, y expr=\thisrow{mode}*-100] {\dat};
    \addplot[gray,fill opacity =0.15] fill between[of=A and B]; 
    
    
    \end{axis}
    \end{tikzpicture}
   
    \caption{Hospital November $11^{th}-12^{th}$, $2021$: three rooms controlled by the GP-MPC controller.}
    \label{fig:hospital}        
 \end{figure}

==> CDC-2022 - Contrasting Data-Driven Techniques/data/Umar.tex <==
 \definecolor{myblue}{rgb}{0.20, 0.6, 0.78}
\definecolor{mygreen}{rgb}{0.2,0.8,0.2}
\definecolor{myred}{rgb}{0.5,0,0}
 \begin{figure}
    \centering
    \begin{tikzpicture}
    \begin{axis}[
    date coordinates in=x,
    % date ZERO=2021-05-13 00:00,   % <-- needs to be set for v1.12 and below
    xmin=2022-02-15 12:00,
    xmax=2022-02-18 08:00,
    % set `xtick distance' to 3 hours (3/24)
    xtick distance=0.5,
    % set the label style of the `xtick's
    % xticklabel=\year.\month.\day\ \hour:\minute]
    xticklabel=\empty,
    % xmin=1, xmax=102,
    ymin=20.9, ymax= 24.2,
    enlargelimits=false,
    clip=true,
    grid=major,
    mark size=0.5pt,
    width=1.05\linewidth,
    height=0.45\linewidth,
    ylabel = {Indoor temperature [$^{\circ} C$]},
    ylabel style={at={(axis description cs:0.085,0.5)}},
    xlabel style={at={(axis description cs:0.5,0.05)}},
    legend columns=3,
    label style={font=\scriptsize},
    ticklabel style = {font=\scriptsize},
    legend style={
    	font=\footnotesize,
    	draw=none,
		at={(0.5,1.03)},
        anchor=south
    } 
    ]
    
    \pgfplotstableread[col sep=comma]{data/UMAR.dat}{\dat};

    \addplot+ [ultra thick,smooth, mark=none, mark options={fill=white, scale=1,line width = 0.1pt},myred] table [x={t}, y={ybar}] {\dat};    
    \addlegendentry{Bang-bang Control};
    \addplot+ [ultra thick,smooth, mark=none, mark options={fill=white, scale=1,line width = 0.1pt},myblue] table [x={t}, y={y}] {\dat};    
    \addlegendentry{DRL Agent};
    \addplot+ [thick,brown,dashed,mark = none,forget plot] table [x={t}, y={ymax}] {\dat};
    \addplot+ [thick,brown,dashed,mark = none] table [x={t}, y={ymin}] {\dat};
    \addlegendentry{Contstraints}
    
    \addplot+ [name path =A, ultra thin, gray,draw opacity=0.6,mark = none] table [x={t}, y expr=\thisrow{mode}*150] {\dat};
    \addplot+ [name path =B, ultra thin, gray,draw opacity=0.6,mark = none] table [x={t}, y expr=\thisrow{mode}*-100] {\dat};
    \addplot[gray,fill opacity =0.15] fill between[of=A and B]; 
    
    
    \end{axis}
    \end{tikzpicture}   
    \begin{tikzpicture}
    \begin{axis}[
    date coordinates in=x,
    % date ZERO=2021-05-13 00:00,   % <-- needs to be set for v1.12 and below
    xmin=2022-02-15 12:00,
    xmax=2022-02-18 08:00,
    % set `xtick distance' to 3 hours (3/24)
    xtick distance=0.5,
    % set the label style of the `xtick's
    % xticklabel=\year.\month.\day\ \hour:\minute]
    xticklabel=\month.\day\ \hour {h},
    % xmin=1, xmax=102,
    ymin=-1, ymax= 103,
    enlargelimits=false,
    clip=true,
    grid=major,
    mark size=0.5pt,
    width=1.05\linewidth,
    height=0.45\linewidth,
    ylabel = {Valve position [$\%$]},
    xlabel= Time,
    ylabel style={at={(axis description cs:0.088,0.5)}},
    xlabel style={at={(axis description cs:0.5,0.05)}},
    legend columns=3,
    label style={font=\scriptsize},
    ticklabel style = {font=\scriptsize}   
    ]
    
    \pgfplotstableread[col sep=comma]{data/UMAR.dat}{\dat};

    \addplot+ [ultra thick,const plot, mark=none, mark options={fill=white, scale=1,line width = 0.1pt},myred] table [x={t}, y expr=\thisrow{ubar}*100] {\dat};    
    \addplot+ [ultra thick,const plot, mark=none, mark options={fill=white, scale=1,line width = 0.1pt},myblue] table [x={t}, y expr=\thisrow{u}*100] {\dat};
    \addplot+ [name path =A, ultra thin, gray,draw opacity=0.6,mark = none] table [x={t}, y expr=\thisrow{mode}*150] {\dat};
    \addplot+ [name path =B, ultra thin, gray,draw opacity=0.6,mark = none] table [x={t}, y expr=\thisrow{mode}*-100] {\dat};
    \addplot[gray,fill opacity =0.15] fill between[of=A and B]; 
    
    
    \end{axis}
    \end{tikzpicture} 
    \caption{UMAR, February $15^{th}-18^{th}$, 2022: one bedroom controlled by a classical rule-based controller (red), the other by the proposed DRL agent (blue). The connection was interrupted in the shaded area and default controllers took over.}
\label{fig:exp_nest}
 \end{figure}

==> CDC-2022 - Contrasting Data-Driven Techniques/data/exp2_min.tex <==
 \definecolor{myblue}{rgb}{0.20, 0.6, 0.78}
\definecolor{mygreen}{rgb}{0.2,0.8,0.2}
\definecolor{myred}{rgb}{0.5,0,0}
 \begin{figure}
    \centering
    \begin{tikzpicture}
    \begin{axis}[
    date coordinates in=x,
    % date ZERO=2021-05-13 00:00,   % <-- needs to be set for v1.12 and below
    xmin=2021-05-13 23:59,
    xmax=2021-05-14 24:00,
    % set `xtick distance' to 3 hours (3/24)
    xtick distance=0.125,
    % set the label style of the `xtick's
    % xticklabel=\year.\month.\day\ \hour:\minute]
    xticklabel=\hour:\minute,
    % xmin=1, xmax=102,
    ymin=5, ymax= 30.5,
    enlargelimits=false,
    clip=true,
    grid=major,
    mark size=0.5pt,
    width=0.9\linewidth,
    height=0.45\linewidth,
    ylabel = {$y$ (indoor temperature [$^{\circ} C$])},
    xlabel= Time,
    ylabel style={at={(axis description cs:0.05,0.5)}},
    xlabel style={at={(axis description cs:0.5,0.05)}},
    legend columns=3,
    label style={font=\scriptsize},
    ticklabel style = {font=\scriptsize},
    legend style={
    	font=\footnotesize,
    	draw=none,
		at={(0.5,1.03)},
        anchor=south
    }    
    ]
    
    \pgfplotstableread[col sep=comma]{data/polydome_min.dat}{\dat}

    \addplot+ [ultra thick,smooth, mark=*, mark options={fill=white, scale=1,line width = 0.1pt},myred] table [x={tt}, y={y}] {\dat};    
    \addlegendentry{Output: y}
    
    \addlegendimage{line legend,ultra thick,smooth, mark=*, mark options={fill=white, scale=1,line width = 0.2pt}, myblue}
    \addlegendentry{Output: u}       
    
    \addplot+ [thick,brown,dashed,mark = none] table [x={tt}, y={max}] {\dat};
    \addplot+ [thick,brown, dashed, mark = none] table [x={tt}, y={min}] {\dat};
    \addlegendentry{Constraint}     
    
    \end{axis}
    
    % ==============================  tracking u
    \begin{axis}[
    axis y line*=right,
    ymin=-0.125, ymax= 3,
    ylabel = {$u$ (Electrical power consumption [$\enspace(kWh)$])},
    axis x line=none,
    date coordinates in=x,
    % date ZERO=2021-05-13 00:00,   % <-- needs to be set for v1.12 and below
    xmin=2021-05-13 23:59,
    xmax=2021-05-14 24:00,
    xtick distance=0.125,
    xticklabel=\hour:\minute,
    enlargelimits=false,
    mark size=0.5pt,
    width=0.9\linewidth,
    height=0.45\linewidth,
    legend style={
    	font=\footnotesize,
    	draw=none,
		at={(0.5,1.00)},
        anchor=south
    },
    ylabel style={at={(axis description cs:1.3,0.5)}},
    legend columns=2,
    label style={font=\scriptsize},
    ticklabel style = {font=\scriptsize}
    ]
    
    \pgfplotstableread[col sep=comma]{data/polydome_min.dat}{\dat}
   
    \addplot+ [ultra thick, mark=*, mark options={fill=white, scale=1.5,line width = 0.2pt}, myblue] table [x={tt}, y expr=\thisrow{u}*0.25] {\dat};
      
    \end{axis} 
    
    \end{tikzpicture}
    \caption{
    \textit{Polydome} $14^{th}$ May 2021: one-day heating with non-robust bilevel data-driven control}
    \label{fig:exp_polydome_2}     
 \end{figure}

==> CDC-2022 - Contrasting Data-Driven Techniques/data/exp3_min_robust.tex <==
\definecolor{myblue}{rgb}{0.20, 0.6, 0.78}
\definecolor{mygreen}{rgb}{0.2,0.8,0.2}
\definecolor{myred}{rgb}{0.5,0,0}
 \begin{figure}
    \centering
        \begin{tikzpicture}
    \begin{axis}[
    date coordinates in=x,
    % date ZERO=2021-05-13 00:00,   % <-- needs to be set for v1.12 and below
    xmin=2021-05-13 23:59,
    xmax=2021-05-14 24:00,
    % set `xtick distance' to 3 hours (3/24)
    xtick distance=0.125,
    % set the label style of the `xtick's
    % xticklabel=\year.\month.\day\ \hour:\minute]
    xticklabel=\empty,
    % xmin=1, xmax=102,
    ymin=5, ymax= 30.5,
    enlargelimits=false,
    clip=true,
    grid=major,
    mark size=0.5pt,
    width=1\linewidth,
    height=0.45\linewidth,
    ylabel = {Indoor temperature [$^{\circ} C$]},
    % xlabel= time,
    ylabel style={at={(axis description cs:0.085,0.5)}},
    xlabel style={at={(axis description cs:0.5,0.05)}},
    legend columns=3,
    label style={font=\scriptsize},
    ticklabel style = {font=\scriptsize},
    legend style={
    	font=\footnotesize,
    	draw=none,
		at={(0.5,1.03)},
        anchor=south
    }    
    ]
    
    \pgfplotstableread[col sep=comma]{data/polydome_min.dat}{\dat}

    \addplot+ [ultra thick,smooth, mark=none, mark options={fill=white, scale=1,line width = 0.1pt},myred] table [x={tt}, y={y}] {\dat};    
    \addlegendentry{System output: y}
    
    \addlegendimage{line legend,ultra thick,smooth, mark=none, mark options={fill=white, scale=1,line width = 0.2pt}, myblue}
    \addlegendentry{Control input: u}       
    
    \addplot+ [thick,brown,dashed,mark = none] table [x={tt}, y={max}] {\dat};
    \addplot+ [thick,brown, dashed, mark = none] table [x={tt}, y={min}] {\dat};
    \addlegendentry{Constraint}     
    
    \end{axis}
    
    % ==============================  tracking u
    \begin{axis}[
    axis y line*=right,
    ymin=-0.125, ymax= 3.2,
    ylabel = {Electrical power [$kWh$]},
    axis x line=none,
    date coordinates in=x,
    % date ZERO=2021-05-13 00:00,   % <-- needs to be set for v1.12 and below
    xmin=2021-05-13 23:59,
    xmax=2021-05-14 24:00,
    xtick distance=0.125,
    xticklabel=\hour:\minute,
    enlargelimits=false,
    mark size=0.5pt,
    width=1\linewidth,
    height=0.45\linewidth,
    legend style={
    	font=\footnotesize,
    	draw=none,
		at={(0.5,1.00)},
        anchor=south
    },
    ylabel style={at={(axis description cs:1.25,0.5)}},
    legend columns=2,
    label style={font=\scriptsize},
    ticklabel style = {font=\scriptsize}
    ]
    
    \pgfplotstableread[col sep=comma]{data/polydome_min.dat}{\dat}
   
    \addplot+ [ultra thick, const plot, mark=none, mark options={fill=white, scale=1.5,line width = 0.2pt}, myblue] table [x={tt}, y expr=\thisrow{u}*0.25] {\dat};
      
    \end{axis} 
    
    \end{tikzpicture}\\
    %\scriptsize{(a)}\\
    \begin{tikzpicture}
    \begin{axis}[
    date coordinates in=x,
    % date ZERO=2021-05-13 00:00,   % <-- needs to be set for v1.12 and below
    xmin=2021-05-24 23:59,
    xmax=2021-05-25 24:00,
    % set `xtick distance' to 3 hours (3/24)
    xtick distance=0.125,
    % set the label style of the `xtick's
    % xticklabel=\year.\month.\day\ \hour:\minute]
    xticklabel=\hour:\minute,
    % xmin=1, xmax=102,
    ymin=5, ymax= 30.5,
    enlargelimits=false,
    clip=true,
    grid=major,
    mark size=0.5pt,
    width=1\linewidth,
    height=0.45\linewidth,
    ylabel = {Indoor temperature [$^{\circ} C$]},
    xlabel= Time,
    ylabel style={at={(axis description cs:0.085,0.5)}},
    xlabel style={at={(axis description cs:0.5,0.05)}},
    legend columns=3,
    label style={font=\scriptsize},
    ticklabel style = {font=\scriptsize},
    legend style={
    	font=\footnotesize,
    	draw=none,
		at={(0.5,1.03)},
        anchor=south
    }    
    ]
    
    \pgfplotstableread[col sep=comma]{data/polydome_min_robust.dat}{\dat}

    \addplot+ [ultra thick,const plot, mark=none, mark options={fill=white, scale=1,line width = 0.1pt},myred] table [x={tt}, y={y}] {\dat};    
    % \addlegendentry{Output: y}
    
    \addlegendimage{line legend,ultra thick,smooth, mark=none, mark options={fill=white, scale=1,line width = 0.2pt}, myblue}
    % \addlegendentry{Output: u}       
    
    \addplot+ [thick,brown,dashed,mark = none] table [x={tt}, y={max}] {\dat};
    \addplot+ [thick,brown, dashed, mark = none] table [x={tt}, y={min}] {\dat};
    % \addlegendentry{Constraint}     
    
    \end{axis}
    
    % ==============================  tracking u
    \begin{axis}[
    axis y line*=right,
    ymin=-0.125, ymax= 3.2,
    ylabel = {Electrical power [$kWh$]},
    axis x line=none,
    date coordinates in=x,
    % date ZERO=2021-05-13 00:00,   % <-- needs to be set for v1.12 and below
    xmin=2021-05-24 23:59,
    xmax=2021-05-25 24:00,
    xtick distance=0.125,
    xticklabel=\hour:\minute,
    enlargelimits=false,
    mark size=0.5pt,
    width=1\linewidth,
    height=0.45\linewidth,
    legend style={
    	font=\footnotesize,
    	draw=none,
		at={(0.5,1.00)},
        anchor=south
    },
    ylabel style={at={(axis description cs:1.25,0.5)}},
    legend columns=2,
    label style={font=\scriptsize},
    ticklabel style = {font=\scriptsize}
    ]
    
    \pgfplotstableread[col sep=comma]{data/polydome_min_robust.dat}{\dat}
   
    \addplot+ [ultra thick,const plot, mark=none, mark options={fill=white, scale=1.5,line width = 0.2pt}, myblue] table [x={tt}, y  expr=\thisrow{u}*0.25] {\dat};
      
    \end{axis} 
    
    \end{tikzpicture}\\
    %\scriptsize{(b)}
    %\caption{\textit{Polydome} one-day heating: (a) $14^{th}$ May 2021: non-robust bilevel data-driven control, (b) $25^{th}$ May 2021: bilevel robust  data-driven  control}
    \caption{\textit{Polydome}. Top: May $14^{th}$, 2021: non-robust bilevel data-driven control. Bottom: May $25^{th}$, 2021: robust bilevel  data-driven  control}
    \label{fig:exp_polydome_3}        
 \end{figure}

==> data/exp2_min.tex <==
 \definecolor{myblue}{rgb}{0.20, 0.6, 0.78}
\definecolor{mygreen}{rgb}{0.2,0.8,0.2}
\definecolor{myred}{rgb}{0.5,0,0}
 \begin{figure}
    \centering
    \begin{tikzpicture}
    \begin{axis}[
    date coordinates in=x,
    % date ZERO=2021-05-13 00:00,   % <-- needs to be set for v1.12 and below
    xmin=2021-05-13 23:59,
    xmax=2021-05-14 24:00,
    % set `xtick distance' to 3 hours (3/24)
    xtick distance=0.125,
    % set the label style of the `xtick's
    % xticklabel=\year.\month.\day\ \hour:\minute]
    xticklabel=\hour:\minute,
    % xmin=1, xmax=102,
    ymin=5, ymax= 30.5,
    enlargelimits=false,
    clip=true,
    grid=major,
    mark size=0.5pt,
    width=0.9\linewidth,
    height=0.45\linewidth,
    ylabel = {$y$ (indoor temperature [$^{\circ} C$])},
    xlabel= Time,
    ylabel style={at={(axis description cs:0.05,0.5)}},
    xlabel style={at={(axis description cs:0.5,0.05)}},
    legend columns=3,
    label style={font=\scriptsize},
    ticklabel style = {font=\scriptsize},
    legend style={
    	font=\footnotesize,
    	draw=none,
		at={(0.5,1.03)},
        anchor=south
    }    
    ]
    
    \pgfplotstableread[col sep=comma]{data/polydome_min.dat}{\dat}

    \addplot+ [ultra thick,smooth, mark=*, mark options={fill=white, scale=1,line width = 0.1pt},myred] table [x={tt}, y={y}] {\dat};    
    \addlegendentry{Output: y}
    
    \addlegendimage{line legend,ultra thick,smooth, mark=*, mark options={fill=white, scale=1,line width = 0.2pt}, myblue}
    \addlegendentry{Output: u}       
    
    \addplot+ [thick,brown,dashed,mark = none] table [x={tt}, y={max}] {\dat};
    \addplot+ [thick,brown, dashed, mark = none] table [x={tt}, y={min}] {\dat};
    \addlegendentry{Constraint}     
    
    \end{axis}
    
    % ==============================  tracking u
    \begin{axis}[
    axis y line*=right,
    ymin=-0.125, ymax= 3,
    ylabel = {$u$ (Electrical power consumption [$\enspace(kWh)$])},
    axis x line=none,
    date coordinates in=x,
    % date ZERO=2021-05-13 00:00,   % <-- needs to be set for v1.12 and below
    xmin=2021-05-13 23:59,
    xmax=2021-05-14 24:00,
    xtick distance=0.125,
    xticklabel=\hour:\minute,
    enlargelimits=false,
    mark size=0.5pt,
    width=0.9\linewidth,
    height=0.45\linewidth,
    legend style={
    	font=\footnotesize,
    	draw=none,
		at={(0.5,1.00)},
        anchor=south
    },
    ylabel style={at={(axis description cs:1.3,0.5)}},
    legend columns=2,
    label style={font=\scriptsize},
    ticklabel style = {font=\scriptsize}
    ]
    
    \pgfplotstableread[col sep=comma]{data/polydome_min.dat}{\dat}
   
    \addplot+ [ultra thick, mark=*, mark options={fill=white, scale=1.5,line width = 0.2pt}, myblue] table [x={tt}, y expr=\thisrow{u}*0.25] {\dat};
      
    \end{axis} 
    
    \end{tikzpicture}
    \caption{
    \textit{Polydome} $14^{th}$ May 2021: one-day heating with non-robust bilevel data-driven control}
    \label{fig:exp_polydome_2}     
 \end{figure}
